Navigation in the Presence of Obstacles for an Agile Autonomous Underwater Vehicle

Navigation underwater traditionally is done by keeping a safe distance from obstacles, resulting in "fly-overs" of the area of interest. Movement of an autonomous underwater vehicle (AUV) through a cluttered space, such as a shipwreck or a decorated cave, is an extremely challenging problem that has not been addressed in the past. This paper proposes a novel navigation framework utilizing an enhanced version of Trajopt for fast 3D path-optimization planning for AUVs. A sampling-based correction procedure ensures that the planning is not constrained by local minima, enabling navigation through narrow spaces. Two different modalities are proposed: planning with a known map results in efficient trajectories through cluttered spaces; operating in an unknown environment utilizes the point cloud from the visual features detected to navigate efficiently while avoiding the detected obstacles. The proposed approach is rigorously tested, both on simulation and in-pool experiments, proven to be fast enough to enable safe real-time 3D autonomous navigation for an AUV.

==> sections/abstract.tex <==
\begin{abstract}
\invis{
During this research project, an efficient method
of underwater navigation with obstacle avoidance was implemented for the AQUA robot. Each of the steps required to
implement this system are explained within this paper and
optimizations within each of the steps are described. This paper
begins by showing the structure of the navigation system and
the ROS nodes which were created in order to enable a motion
tree based approach. The next section describes the method of
generating a motion tree as well as an optimization through
the translation of the motion tree. After this, the methods
used to detect obstacles and select paths are covered. The end
of the paper consists of a review of the effectiveness of the
implemented navigation system, an analysis of its efficiency,
and a discussion of future optimization.
}
\end{abstract}


==> sections/experiments.tex <==
\section{EXPERIMENTS}
\label{sec:exp}
\begin{figure*}[th]
\begin{center} 
\leavevmode
\begin{tabular}{cc}
\subfigure[]{\includegraphics[height=1.6in]{figures/room_sideview_alt}\label{fig:pool3_side}}&
\subfigure[]{\includegraphics[height=1.6in]{figures/room_topview_alt}\label{fig:okvis}}\\
\subfigure[]{\includegraphics[height=1.5in]{figures/aqua_pool2_sideview}\label{fig:okvis}}&
\subfigure[]{\includegraphics[height=1.5in]{figures/aqua_pool2_topview}\label{fig:okvis}}\\
\subfigure[]{\includegraphics[height=1.45in]{figures/pool5_sideview}\label{fig:svind}} &
\subfigure[]{\includegraphics[height=1.45in]{figures/pool5_topview}\label{fig:svind}} 
\end{tabular}
\end{center}
   \caption{Simulated trajectories executed by the robot in Gazebo. (a-b) show a side and top perspective of the Window environment (the ceiling is not shown for the top view). (c-d) show the Pipes environment. Finally (e-f) show the Cluttered environment}
   \label{fig:comparison}
 \end{figure*}

\textcolor{red}{N: is this from the previous paper???}


\subsection{Simulation}
Multiple challenging environments were created aiming to test the capability of the Aqua2 to overcome drifting, to successfully avoid the obstacles, to follow reasonable paths, and to surpass the local minimum problems expected to occur in man-made environments with Trajopt. The executed paths for these environments are shown in Fig.~\ref{fig:comparison}.



The second environment, called the Pipes Environment, is intended to test the ability of the Aqua2 to safely maneuver through an environment that requires a 3D motion and consecutive change on yaw, pitch and roll. It can be observed that the robot moves around the obstacles while keeping the safety distance. 
Trajopt produced naturally also the roll orientation that reduced the drift, smoothing the motion. 
Such behaviour intuitively could be explained by understanding the bounded distance optimization of the swept-out volumes between two states. A rotation is expected to occur when an obstacle is in proximity, and the roll will be adjusted so that during the motion the robot will be perpendicular to the normal of the obstacle, thus naturally reducing the drag.





\subsection{Pool Trials}
\begin{figure}[h]
{\includegraphics[width=\columnwidth]{./figures/AquaPoolTop1-resized}}
\smallskip\\
{\includegraphics[width=\columnwidth]{./figures/pool3_sideview}}
\caption{Aqua2 AUV during deployment in the pool and a side view of the path as executed in the simulation.}
\label{fig:poolOver}
\end{figure}


\begin{figure*}[h]
\begin{center}
\leavevmode
\begin{tabular}{ccc}
 \subfigure[]{\includegraphics[height=1.25in]{figures/pool3_topview}\label{fig:pool3_top}}&
  \subfigure[]{\includegraphics[height=1.36in]{figures/Pool1}\label{fig:pool1}}&
\subfigure[]{\includegraphics[height=1.36in]{figures/Pool2}\label{fig:pool2}}\\
 \subfigure[]{\includegraphics[height=1.36in]{figures/Pool3}\label{fig:pool3}}&
  \subfigure[]{\includegraphics[height=1.36in]{figures/Pool4}\label{fig:pool4}}&
\subfigure[]{\includegraphics[height=1.36in]{figures/Pool5}\label{fig:pool5}}
\end{tabular}
\end{center}
   \caption{Top-down view of the executed path in Gazebo with representative photos from the real deployment in the pool.}
   \label{fig:experiment}
 \end{figure*}

\invis{
\mcomment{???}
A number of experiments were conducted in a 25m long and 4m deep pool, where artificial obstacles were placed to simulate a complicated obstacle rich environment. Prior to testing obstacle avoidance extensive testing was performed to build a library of motions that aqua is able to execute smoothly. One of the main observations was that when changing the relative angle of robot, strict threshold might result in overshooting and very complicated behavior. All this is caused by the complexity of complicated dynamics of the environment. ...\mcomment{???}
}


 One of the future plans is to use the  Aqua2 for shipwreck inspection and to study online state estimation in deep underwater environments, where most of the features are likely to be at the bottom. For this purpose a constraint was added to not allow roll rotations during the motion in order to keep the stereo cameras facing the floor. A similar environment to the Poles was used, with the exception that due to the expected larger drifting effect, the last pole was slightly moved further as shown in the executed path of the Gazebo simulation in Fig.~\ref{fig:pool3_side} and Fig~\ref{fig:pool3_top}. The IMU and the depth sensor were used to guide the robot through the pool trials. The robot travelled 15m across the pool avoiding the obstacles. Fig~\ref{fig:pool1} through Fig~\ref{fig:pool5} present representative snapshots of the robots behaviour. 

\invis{
It should be disclosed that although the Aqua2 had to swim for 15 meters to reach the goal and state estimation was not deployed to provide accurate positioning, the robot using only the IMU, the depth sensor and prerecorded odometry from simulation, it was able to safely navigate around the obstacles accurately validating the path length and safety guaranties of the proposed approach. }






==> sections/introduction.tex <==
\section{INTRODUCTION}\pagebudget{1}

%Key phrase: sampling-based correction

This paper addresses the problem of trajectory planning for underwater structure inspection and mapping.
Underwater structure mapping is an important capability applicable to multiple domains: marine archaeology, infrastructure maintenance, resource utilization, security, and environmental monitoring. 
While the proposed approach is not limited to the underwater domain, this work addresses the challenging conditions encountered underwater, with a special focus on shipwreck mapping. 
Historical shipwrecks tell an important part of history and at the same time have a special allure for most humans, as exemplified by the plethora of movies and artworks of the Titanic; see the work of Eustice et al.~\cite{eustice2006visually} for the visual mapping of the Titanic.
Underwater mapping has traditionally focused on acoustic sensors~\cite{gary20083d,johannsson2010imaging,teixeira2018multibeam,przeslawski2018comparative}, however, most inspections require visual input~\cite{abadie2018georeferenced,drap2012underwater,figueira2015accuracy}. The state\hyp of\hyp the\hyp art in autonomous operations is to observe the target structure from far enough to avoid navigation in cluttered spaces, while remotely controlled operations present entanglement hazards. As a result most inspections suffer from gaps due to occlusions, and low\hyp resolution due to the water effects on the camera sensor. The  presented  work will enable autonomous operations underwater close to the structure to be inspected; this was only partially possible with teleoperation before.

Maps of underwater structures such as wrecks, caves, dams, and docks are often available either through acoustic sensing~\cite{leonard2012directed} or via photogrammetry~\cite{menna2018photogrammetric,agrafiotis2018underwater}. In this paper we present an adaptation of the Trajopt~\cite{schulman2013finding} open source package for an 3D trajectory planning of an AUV in a known map, realized on an Aqua2 vehicle~\cite{Rekleitis2005d}. The Trajopt planner was augmented with a sampling\hyp based correction scheme that resolved the local minima challenge. Furthermore, different map representations were tested including geometric primitives and point\hyp cloud implementations.  

\begin{figure}
\includegraphics[width=\columnwidth]{./figures/Speedo1Stav-resized}
\caption{Aqua2 AUV navigating over the Stavronikita shipwreck, Barbados.}
\label{fig:beauty}
\end{figure}

AUVs moving in 3D underwater are prone to external forces, such as currents, and also the effects of inertia. As such, when a robot switches between motion directions, a significant drift appears. This effect was taken into consideration when designing the safety distance and the linear velocity of the vehicle. When the motions were too aggressive, excessive drift was observed. Utilizing a complete hydrodynamics model of the Aqua2 would lead to resolving such issues, such a model has yet to be introduced. Previous works~\cite{georgiades2009simulation,giguere2006characterization,plamondon2008trajectory} attempted to provide such analysis but they were restricting significantly the mobility of the robot since it was allowed to turn only by no more than one axis each time. The above makes it infeasible to directly account also for the dynamics during planning. It is worth to note though, that fast motion planners, such as KPIECE~\cite{csucan2009kinodynamic} that are using physics simulators to plan with kinodynamic constraints can solve the planning problems for systems with non-trivial dynamics. But the fact that the Aqua2 hexapod robot has a very large control space, limited computing resources to accommodate for  physics simulators operating in parallel, and non trivial task-depended projections --required by KPIECE~\cite{csucan2009kinodynamic}-- the use of such techniques requires excessive resources for a real-time response. 

A variety of environments were constructed to challenge the trajectory generator. Utilizing the gazebo simulator \cite{koenig2004design} with an underwater extension that emulates the kinematic behaviour of the Aqua2 vehicle, the tested environments demonstrated changes in depth, and attitude in three dimensions for realizing the produced trajectories. Furthermore, tests in our university's diving pool, with different obstacle setups verified the validity of the proposed approach. The obstacle arrangements in the pool were accurately reproduced with a map which was used as input to the Trajopt planner. 

In summary the contribution of this paper is triple:
\begin{itemize}
    \item Trajopt, a popular path optimization package for manipulators, was extended for 3-D path planning of mobile robots, and functionality was added for convex decomposition of unordered point-clouds. Additionally, a new sampling-based method producing diverge paths was introduced for fast warm restarting to avoid local minima issues.
    \item Using the above modifications a novel, yet simple, light-weight geometric navigation framework that utilizes fully 3D motion capabilities, is introduced, for underwater vehicles with lack of a complete hydro-dynamics analysis. The framework guarantees minimum clearance to account for oscillations.  
    \item The proposed method is used to enable autonomous 3-D navigation, for the first time, for the Aqua2 hexapod underwater robot with both off-line and on-line planning. Moreover for online planning a vision based navigation framework was introduced with real-time replanning of $2$ Hz, with using limited on-board computing resources, working in parallel with a computationally demanding underwater SLAM package, SVIN~\cite{RahmanICRA2018}. The robot is shown to be able to navigate safely in challenging environments of substantial complexity, with respect to other studies in the past, even without utilizing a known hydro-dynamics model.
\end{itemize}

The next section provides an overview of related work. Section \ref{sec:system} describes the Aqua2 AUV employed. The proposed approach is detailed in Section \ref{prop_meth}, while experimental results are presented in Section \ref{sec:exp}. The paper concludes with lessons learned and directions of future work.


==> sections/litreview.tex <==
\section{RELATED WORK}\pagebudget{0.5}
\label{ch:litReview}

The underwater domain introduces additional complexities to path planning.  In such highly dynamic environments one of the main challenges is to generate a safe path .  Several methods have been explored to correct the deviations caused by currents, including the FM* planning system~\cite{petres2007path}. Other methods rely on observations about the structure of the terrain~\cite{williams2001towards} and satellite imagery~\cite{garau2009path} to estimate the effects of currents. Genetic algorithms \cite{alvarez2004evolutionary} and mixed integer linear programming approaches \cite{yilmaz2008path} have also been used to support the computation of paths in dynamic underwater environments.

Recent works, such as the one by Hernandez, Vidal, et al.~\cite{hernandez2019online} provided an on-line sampling based framework for an AUV in 3D accounting also for the dynamics of the system. The proposed framework although was shown to be capable to work in real-time, even for trivial examples offline, it needed close to half a minute for producing solutions with clearance guarantees. Moreover during the on-line experiments the replanning was close to 1Hz but the robot was constrained to a constant depth reducing the planning space to 2D. When it comes to accounting also for currents, other studies~\cite{lee2017energy,vidal2019online} are using sampling\hyp based techniques utilizing a complete dynamic model of the AUV, but are shown to work only in trivial environments with few obstacles.

Another challenge in underwater path planning is to generate paths fast enough to be able to compute and execute them online. Green and Kelly demonstrated a branching\hyp based method for quickly generating safe paths in 2D environment  \cite{green2007toward} which has since been the basis of several optimizations  \cite{knepper2009empirical, knepper2012real, pivtoraiko2009differentially, branicky2008path}. Path planning has also been optimized by reducing candidate paths to equivalence classes \cite{knepper2012toward}.

Optimal sampling\hyp based techniques~\cite{karaman2010incremental, gammell2014informed, janson2015fast, gammell2015batch} although provide near-optimal solutions and have improved with time, in general require more resources, more time, and often an exhaustive search of the configuration space. In addition, it is very challenging for these techniques to satisfy minimum distances from the obstacles. Some studies on online underwater navigation with sampling-based techniques provide quickly with safe paths, however they are limited to 2D motions~\cite{hernandez2016planning} or require assumptions for vertical relief~\cite{vidal2018online} without exploiting the full potential of performing 3D motions. 

In some applications it is often necessary for AUVs to navigate in an environment without global knowledge of the environment. In such cases, obstacles are observed, often by stereo vision as has been done on aerial vehicles \cite{zhu20163d}. Exploration of an unknown environment by aerial vehicles has been represented using a 3D occupancy grid using probabilistic roadmaps (PRM) and the D* Lite algorithm for planning \cite{hrabar20083d}. Although underwater and aerial domains provide different challenges, both require path planning in 3D. For an AUV such as Aqua2 whose movements do not correlate exactly with control inputs, planning becomes even more difficult. Other AUVs have also been used for path planning, such as RAIS~\cite{antonelli2001real} and DeepC~\cite{eichhorn2005reactive}. Another AUV, REMUS~\cite{fodrea2003obstacle}, used obstacle avoidance specifically for exploration of shallow waters.

Enabling Aqua2 AUVs to perform complex tasks has been attempted few times. The lack of a complete hydro-dynamics model of the robot of underwater navigation is more challenging and presented works in the previous paragraphs have yet to propose an alternative sufficient solution for such systems. At the beginning basic patterns were used, then complex swimming gaits were developed in order to perform patterns such as swimming on the side, in a corkscrew motion, or performing a barrel roll~\cite{meger2015learning}, and enabled the robot to move reactively. Visual tags placed on structures were used to enable the AUV to navigate~\cite{6942867}, while a learned reactive controller had the vehicle maintain a safe distance while moving over a coral reef~\cite{Manderson2018_oceans,Manderson2018}. 

% Navigation in 3D in unknown environment using AUV. Stereo vision is used for obstacle detection. Path planning is based on PRM and D* Lite. The environment is represented with 3D occupancy grid \cite{hrabar20083d}. 
% Collision avoidance in dynamic environment with AUV \cite{zhu20163d}. Motion primitives and 3D motion planning \cite{paranjape2015motion}





==> sections/problStat.tex <==
\section{System Overview}\label{sec:system}





==> sections/proposedMethods.tex <==
\section{Proposed Method}
\label{prop_meth}




\subsection{Motion planner}\label{sec:mp}





%
The next few sections describe the specific adaptations made to Trajopt to achieve strong performance in this domain.

\subsubsection{Forming an effective cost function}




\subsubsection{Sampling-based corrections for optimization  local minima}\label{sec:correct}


\subsubsection{Map representations}
 
 







\subsection{Path Tracker}\label{sec:control}





